Black-Box Strategies and Equilibrium for Games with Cumulative Prospect Theoretic Players

The betweenness property of preference relations states that a probability mixture of two lotteries should lie between them in preference. It is a weakened form of the independence property and hence satisfied in expected utility theory (EUT). Experimental violations of betweenness are well-documented and several preference theories, notably cumulative prospect theory (CPT), do not satisfy betweenness. We prove that CPT preferences satisfy betweenness if and only if they conform with EUT preferences. In game theory, lack of betweenness in the players' preference relations makes it essential to distinguish between the two interpretations of a mixed action by a player - conscious randomizations by the player and the uncertainty in the beliefs of the opponents. We elaborate on this distinction and study its implication for the definition of Nash equilibrium. This results in four different notions of equilibrium, with pure and mixed action Nash equilibrium being two of them. We dub the other two pure and mixed black-box strategy Nash equilibrium respectively. We resolve the issue of existence of such equilibria and examine how these different notions of equilibrium compare with each other.

==> tex/mediatedeq.tex <==
%!TEX root = ../main.tex

\section{Correlated and Mediated equilibrium}


To define a BB CPT correlated equilibrium, let $\phi \in \Delta_f(S)$ denote a mediator distribution. Let $\phi_i[\cdot]$ denote the marginal distribution on $\Delta_f(S_i)$ and $\phi_{-i}[\cdot|s_i]$, the conditional distribution given $s_i \in \supp \phi_i[\cdot]$. Mediator samples $s = (s_i)_{i \in N}$ from the distribution $\phi$. Player $i$ computes the conditional distribution $\phi_{-i}[\cdot|s_i] \in \Delta_f(S_{-i})$ which further induces a distribution $\mu_{-i}(\phi_{-i}[\cdot|s_i]) \in \Delta(A_{-i})$. 

\begin{definition}
	A mediator distribution $\phi$ is a BB CPT CE iff for all $i$ and all $s_i \in \supp (\phi_i)$ we have
	\[
		s_i \in BR_i(\mu_{-i}(\phi)[\cdot|s_i]).
	\]
\end{definition}

\begin{proposition}
	A mediator distribution with product form, $\phi = \sigma$, is BB CPT CE iff it is BB CPT NE.
\end{proposition}

We now define the BB CPT mediated equilibrium notions. Suppose we add a signal system $(B_i)_{i \in N}$ to a game $\Gamma$, where each $B_i$ is a finite set. Suppose there is a mediator who sends a signal $b_i \in B_i$ to player $i$. 
Let $B = \Pi_{i \in N} B_i$ be the set of all signal profiles $b = (b_i)_{i \in N}$ and $B_{-i} = \Pi_{j \neq i} B_j$ denote the set of signal profiles $b_{-i}$ of all players except player $i$.
%Let $\tilde \Gamma = (\Gamma, (B_i)_{i \in N})$ denote such a game with signal system. We call it a \emph{mediated game}.
The mediator is characterized by a distribution $\psi \in \Delta(B)$.
 %that we call the \emph{mediator distribution}. 
 Thus, the mediator draws a signal profile $b = (b_i)_{i \in N}$ from the mediator distribution $\psi$ and sends signal $b_i$ to player $i$.
%In the definition of a correlated equilibrium the set $B_i$ is restricted to the set of actions $A_i$ for each player $i$.

A \emph{mediated BB strategy} for any player $i$ is given by a function $\strat_i : B_i \to \Delta(S_i)$ and a \emph{mediated BB strategy profile} $\strat = (\strat_1,\dots,\strat_n)$ gives the mediated BB strategy for all players. 
We define the \emph{best response set} of player $i$ to a mediated BB strategy profile $\strat$ and a mediator distribution $\psi$ as
\begin{align}
\label{eq: best_response}
	BR_i^{\psi} (\strat_{-i}) := \bigg\{ \strat^*_i &: B^i \to \Delta_f(S_i) \bigg| \text{ for all } b_i \in B_i \nonumber\\
	& \supp(\strat^*_i(b_i)) \subset BR_i(\tilde \mu_{-i}(a_{-i}|b_i)) \bigg\}
\end{align}
where
\begin{equation}
\label{eq: tilde_mu}
	\tilde \mu_{-i}(a_{-i} | b_i ) := \sum_{b_{-i} \in B_{-i}} \psi_{-i}(b_{-i}|b_i) \sum_{s_{-i} \in \strat_{-i}(b_i)} \prod_{j \neq i} \strat_j(b_j)[s_j] \prod_{j \in N \back i} s_j(a_j).
\end{equation}
and $\supp(\cdot)$ denotes the support of the distribution within the brackets.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{definition}
 A mediated BB strategy profile $\strat$ is said to be a \emph{mediated BB CPT Nash equilibrium} of a game $\Gamma$ with respect to a mediator distribution $\psi \in \Delta(B)$ iff
	\[
		\strat_i \in BR_i^{\psi}(\strat_{-i})  \text{ for all } i \in N.
	\]
%Let $\Sigma(\Gamma, (B_i)_{i \in N}, \psi)$ denote the set of all mediated CPT BB Nash equilibria of $\Gamma$ with respect to a mediator distribution $\psi \in \Delta(B)$.
\end{definition}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

For any mediator distribution $\psi \in \Delta(B)$, and any mediated BB strategy profile $\strat$, let $\eta(\psi,\strat) \in \Delta(S)$ be given by
\begin{equation}
\label{eq: eta_def}
	\eta(\psi,\strat)(s) := \sum_{b \in B} \psi(b) \prod_{i \in N} \strat_i(b_i)[s_i].
\end{equation}	

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
